Large-Scale Meta-Learning with Continual Trajectory Shifting

Meta-learning of shared initialization parameters has shown to be highly effective in solving few-shot learning tasks. However, extending the framework to many-shot scenarios, which may further enhance its practicality, has been relatively overlooked due to the technical difficulties of meta-learning over long chains of inner-gradient steps. In this paper, we first show that allowing the meta-learners to take a larger number of inner gradient steps better captures the structure of heterogeneous and large-scale task distributions, thus results in obtaining better initialization points. Further, in order to increase the frequency of meta-updates even with the excessively long inner-optimization trajectories, we propose to estimate the required shift of the task-specific parameters with respect to the change of the initialization parameters. By doing so, we can arbitrarily increase the frequency of meta-updates and thus greatly improve the meta-level convergence as well as the quality of the learned initializations. We validate our method on a heterogeneous set of large-scale tasks and show that the algorithm largely outperforms the previous first-order meta-learning methods in terms of both generalization performance and convergence, as well as multi-task learning and fine-tuning baselines.

==> sections/ablation.tex <==
\begin{table}[t]
\vspace{-0.1in}
\centering
\small
  \caption{\small\textbf{Ablation study.}}
  \vspace{0.05in}
 \begin{tabular}{c | c c}
 \hline
 & \multicolumn{2}{c}{Target Dataset} \\
 Model & Stanford Cars & STL10  \\
 \hline
 \hline
No correction
& xx.xx\tiny$\pm$x.xx
& xx.xx\tiny$\pm$x.xx \\

Random correction 
& xx.xx\tiny$\pm$x.xx
& xx.xx\tiny$\pm$x.xx \\

No resetting
& xx.xx\tiny$\pm$x.xx
& xx.xx\tiny$\pm$x.xx \\

\hline

\bf Ours 
& \bf xx.xx\tiny$\pm$x.xx
& \bf xx.xx\tiny$\pm$x.xx \\
\hline
\end{tabular}
  \label{tbl:ablation}
\end{table}

==> sections/approach_bkup.tex <==
\section{Approach}
\label{approach}
In this section, we first describe a form of parameter amortization. Then, we explain about computation of meta-gradient and propose a corresponding meta-learning framework.
% In this section, we introduce meta-learning framework via amortization that is scalable to large-scale tasks. 
% For scalable meta-learning, reqwe need to consider,

% We describe parameter amortization function and training scenario. 

\subsection{Parameter amortization}
% The conventional transfer learning method transfers parameters assuming optimal parameter space is shared across tasks, which is not always correct. To consider difference between parameter space, we propose an parameter amoriztation function as a mapping between parameter spaces. 
Flennerhag et al.~\cite{}, Lee et al.~\cite{} and Park et al.~\cite{} propose an approximation of meta-gradient using preconditioning gradient. However, those methods lack consideration for task heterogeneity, since they share initialization and preconditioning method for every tasks. To consider task heterogeneity, we propose paramter amortization that generates task-specific initialization and plays a little role of preconditioning gradient. 
In detail, we design an amortization with affine transformation, where parameters for affine transformation is obtained from task set encoding. Formally, when task $\tau$ is given, task-specific parameter is generated as  
% the entire set or a subset of the main network parameters $\theta$. However such parameter transfer may become ineffective when we transfer knowledge across a dissimilar pair of source and target tasks. Thus, we propose to amortize parameter to obtain task-specific parameter. For simplicity, we set amortization function $f$ with affine transformation as follows.
\[\theta_\tau=f(\theta, \tau;\phi)=(1+\gamma)\cdot\theta+\beta \quad \textrm{where} \quad g(\tau;\phi) = [\gamma;\beta]\]

The reasons for using affine transformation are (1) it is simple but flexible enough to represent mapping and (2) can provide simple form for algorithm. The detail of (2) will be described in the next section.

\subsection{Training of amortization function}
% To train the amortization function, proper objective is required. 
Next, we propose an objective to train the amortization function, $f(\theta, \tau;\phi)$. Our goal is that task-specific parameter obtained by amortization performs well on the target task, even without further inner gradient steps. Hence, we can set task loss with the amortized parameter, i.e. $\mathcal{L}_{\theta_\tau^{(0)}}$, as an objective for training amortization function parameter. Note that, amortization is a function on network parameter and gradient over network parameter is required. In practice, however, tracking gradient over network parameters is not easy within the famous deep learning frameworks, such as TensorFlow or pytorch. Thus, we propose regression loss from $f(\theta, \tau;\phi)$ to $\theta_\tau^{(1)}$, i.e. parameter after a gradient step, as an objective, that can be derived from following lemma.

\begin{lemma}
    % Let $\theta_i^{(0)}=f(\theta, \mathcal{D}_i;\phi)$ be an amortized parameter for task $\mathcal{T}_i$ and $\theta_i^{(1)}$ be a parameter after a single gradient step from $\theta_i^{(0)}$, using SGD-based update. 
    Assume that, we perform inner gradient step with SGD-based update. Then, optimization with objective $\left(f\left(\theta, \tau;\phi\right)-\theta_\tau^{(1)}\right)^2$, i.e. regression MSE loss from $f(\theta, \tau;\phi)$ to $\theta_\tau^{(1)}$ is as same as optimization with objective $\mathcal{L}_{\theta_\tau^{(0)}}$,  i.e. task loss of amortized parameter.  
\end{lemma}

\begin{proof}
Using SGD-based update, 
\begin{equation}
    \label{eqn:1}
    \theta_\tau^{(1)}\approx \theta_\tau^{(0)}-\alpha\cdot\nabla_{\theta_\tau^{(0)}}\mathcal{L}_{\theta_\tau^{(0)}},
\end{equation}
 with some learning rate $\alpha$.
For optimization with objective $\mathcal{L}_{\theta_\tau^{(0)}}$, gradient for $\phi$ is calculated as
\begin{equation}
        \nabla_{\phi}\mathcal{L}_{\theta_\tau^{(0)}}=\nabla_{\theta_\tau^{(0)}}\mathcal{L}_{\theta_\tau^{(0)}}\cdot \nabla_{\phi}{\theta_\tau^{(0)}}
\end{equation}
, using chain rule. Substituting $\nabla_{\theta_\tau^{(0)}}\mathcal{L}_{\theta_\tau^{(0)}}$ through (\ref{eqn:1}),
\begin{align}
    \nabla_{\phi}\mathcal{L}_{\theta_\tau^{(0)}}&=\frac{(\theta_\tau^{(0)}-\theta_\tau^{(1)})}{\alpha}\cdot \nabla_{\phi}{\theta_\tau^{(0)}} \\
    &= \frac{1}{2\alpha}\cdot\nabla_{\phi}\left(\theta_\tau^{(0)}-\theta_\tau^{(1)}\right)^2\\
    &\propto \nabla_{\phi}\left(f(\theta, \tau;\phi)-\theta_\tau^{(1)}\right)^2
\end{align}
Therefore, optimization with regression MSE loss from $f(\theta, \tau;\phi)$ to $\theta_\tau^{(1)}$ is as same as optimization with task loss of $\theta_\tau^{(0)}$. 
% \begin{align}
%     \nabla_{\phi}\mathcal{L}_{\theta_i^{(0)}}&=\nabla_{\theta_i^{(0)}}\mathcal{L}_{\theta_i^{(0)}}\cdot \nabla_{\phi}{\theta_i^{(0)}}\\
%     % &=\nabla_{\theta_i^{(0)}}\mathcal{L}_{\theta_i^{(0)}}\cdot \nabla_{\phi}f(\theta, \mathcal{D}_i;\phi)
% \end{align}
% , via chain rule. From \ref{eqn:1}, 
\end{proof}

For updating base parameter $\theta$, we first apply inverse-amortization $f^{-1}$ to task-specific updated parameters, and interpolate between averaged updated parameters and original parameter. Formally, 
\[\theta \leftarrow \theta + \beta\cdot\left(\frac{1}{|\mathcal{T}|}\sum_{\tau \in \mathcal{T}}f^{-1}(\theta_\tau^{(1)}) - \theta\right)\]
This is also equivalent to using task loss of amortized parameter, i.e. $\mathcal{L}_{\theta_\tau^{(0)}}$, when $f$ is defined as an affine transformation.

% \begin{lemma}
%     When $f$ is a function of form $f(\theta, \tau;\phi)=(1+\gamma)\cdot\theta+\beta$, optimization of $\theta$ with task loss $\mathcal{L}_{\theta_\tau^{(0)}}$ can be done with 
%     \[\theta \leftarrow \frac{1}{|\mathcal{T}|}\sum_{\tau \in \mathcal{T}}f^{-1}(\theta_\tau^{(1)})\]
% \end{lemma}

% \begin{proof}
% For optimization with objective $\mathcal{L}_{\theta_\tau^{(0)}}$, gradient for $\theta$ is calculated as
% \begin{equation}
%         \nabla_{\theta}\mathcal{L}_{\theta_\tau^{(0)}}=\nabla_{\theta_\tau^{(0)}}\mathcal{L}_{\theta_\tau^{(0)}}\cdot \nabla_{\theta}{\theta_\tau^{(0)}}
% \end{equation}
% , using chain rule. Substituting $\nabla_{\theta_\tau^{(0)}}\mathcal{L}_{\theta_\tau^{(0)}}$ through (\ref{eqn:1}),
% \begin{align}
%     \nabla_{\theta}\mathcal{L}_{\theta_\tau^{(0)}}&=\frac{(\theta_\tau^{(0)}-\theta_\tau^{(1)})}{\alpha}\cdot \nabla_{\theta}{\theta_\tau^{(0)}} \\
%     &= \frac{(1+\gamma)\cdot\theta+\beta-\theta_\tau^{(1)}}{\alpha}\cdot(1+\gamma)\\
%     &\propto \nabla_{\phi}\left(f(\theta, \tau;\phi)-\theta_\tau^{(1)}\right)^2
% \end{align}
% Therefore, optimization with regression MSE loss from $f(\theta, \tau;\phi)$ to $\theta_\tau^{(1)}$ is as same as optimization with task loss of $\theta_\tau^{(0)}$. 
% % \begin{align}
% %     \nabla_{\phi}\mathcal{L}_{\theta_i^{(0)}}&=\nabla_{\theta_i^{(0)}}\mathcal{L}_{\theta_i^{(0)}}\cdot \nabla_{\phi}{\theta_i^{(0)}}\\
% %     % &=\nabla_{\theta_i^{(0)}}\mathcal{L}_{\theta_i^{(0)}}\cdot \nabla_{\phi}f(\theta, \mathcal{D}_i;\phi)
% % \end{align}
% % , via chain rule. From \ref{eqn:1}, 
% \end{proof}
% In other word, task loss with the amortized parameter, should be sufficiently small. Let's denote amortized parameter with $\theta_i^{(0)}=f(\theta, \mathcal{D}_i;\phi)$. Then, 
\subsection{Algorithm}
Using above explanation, final algorithm for training amortization function and base parameter is as follows:
\begin{algorithm}[H]
	\caption{Meta-training}\label{algo:algorithm1}
	\small
	\begin{algorithmic}[1]
	\State \textbf{Base parameter}: $\theta$, \textbf{Amortization for task $\tau$}: $f(\theta,\tau;\phi)$
% 		\State \textbf{Input:} $(\D_1^\tr,\D_1^\te),\dots,(\D_T^\tr,\D_T^\te)$
% 		\State \textbf{Input:}
% 		Learning rate $\alpha$
% 		\State \textbf{Output:} $\theta^*, \phi^*$
		\State Randomly initialize $\theta$, $\phi$ %, \psi_1,\dots,\psi_T$.
		\While{not converged}
		\For{$\tau \in p(\mathcal{T})$}
		\State $\theta_\tau^{(0)} \leftarrow f(\theta,\tau;\phi)$
		\Comment Amortization
% 		\State Compute $\mathcal{L}_i^{(0)}$ with $\theta_t^{(0)}$.
		\State Update $\theta_t$ with $k$ steps of SGD.
% 		\State {Sample $\mathcal{B}_t^\tr \subset \D_t^\tr$}.
% 		\State Compute $\mathcal{L}^{\tr}=\mathcal{L}(\mathcal{D}_t^\tr;\theta_t^{(0)}, \psi_t)$.
% 		\State $\theta_{t} \leftarrow \theta_t - \alpha \grad_{\theta} \mathcal{L}^\tr$ %(\mathcal{B}_t^\tr;\theta,\phi, \psi_t)$	
% 		\State $\psi_{t} \leftarrow \psi_t - \alpha \grad_{\psi_t} \mathcal{L}^{tr}$ %(\mathcal{B}_t^\tr;\theta,\phi, \psi_t)$
% 		\State Compute $\mathcal{L}^{te}_t = \mathcal{L}(\mathcal{B}_t^\te;\theta, \psi_t)$ for $t=1\cdots T$.
		\EndFor
		\State $\phi \leftarrow \phi -\alpha\frac{1}{|\mathcal{T}|}\sum_{\tau \in p(\mathcal{T})}\nabla_\phi\left(f\left(\theta, \tau;\phi\right)-\theta_\tau^{(1)}\right)^2$
		\State $\tilde\theta \leftarrow \frac{1}{|\mathcal{T}|}\sum_{\tau \in p(\mathcal{T})}f^{-1}(\theta_\tau)$
		\Comment{Inverse amortization} %(\mathcal{B}_t^\te;\theta,\phi, \psi_t)$
		\State $\theta  \leftarrow \theta + \beta(\tilde\theta-\theta)$
		\Comment Update shared theta
		

% 		\State $\phi \leftarrow \phi - \alpha \grad_{\phi} \frac{1}{T}\sum_{t=1}^{T} \mathcal{L}^{te}_t$
% 		\Comment{update $\phi$ with test data}
		\EndWhile
	\end{algorithmic}
	\end{algorithm}
	
	\begin{algorithm}[H]
	\caption{Meta-testing}\label{algo:algorithm2}
	\small
	\begin{algorithmic}[1]
% 		\State \textbf{Input:} $\D^\tr,\theta^*, \phi^*$
% 		\State \textbf{Input:} Learning rate $\alpha$
% 		\State \textbf{Input:} $\phi^*$
% 		\State \textbf{Output:} $\theta^*, \psi^*$
        \State \textbf{Converged parameters}: $\theta^*, \phi^*$, \textbf{Target task}: $\tau$
		\State $\theta_\tau \leftarrow f(\theta^*, \tau;\phi^*)$
% 		\State Randomly initialize $\psi$.
% 		\State Initialize $\theta$ with $\theta^*, \psi^*$
		\While{not converged}
		    \State Fine-tune $\theta_\tau$ with $\mathcal{D}_\tau$
% 		\State Sample $\mathcal{B}^\tr \subset \D^\tr$.
% 		\State Compute $\mathcal{L}^{tr} = \mathcal{L}(\mathcal{B}^\tr;\theta^*, \psi)$. %noise sampling.
% 		\State $\theta \leftarrow \theta - \alpha \grad_{\theta} \mathcal{L}^\tr$
% 		\State $\psi \leftarrow \psi - \alpha \grad_{\psi} \mathcal{L}^\tr$  %(\mathcal{B}^\tr;\theta^*,\phi^*, \psi)$
		\EndWhile
% 		\State $\theta^* \leftarrow \theta$
		%\State Sample $S$ Monte-Carlo samples for the test examples in $\mathcal{D}^\te$.
% 		\State Evaluate the test examples in $\D^\te$ with MC approximation and the parameter $\theta^*$.
% 		\State
% 		\State
	\end{algorithmic}
	\end{algorithm}
	
	
\newpage
% Following notations from Reptile~\cite{}, let's denote
% \begin{align*}
%     \mathcal{L}_i& &&: i\text{-th task loss}\\
%     % g_i&=\nabla_{\phi_i}\mathcal{L}_i&&: i\text{-th gradient obtained during SGD}\\
%     g_i&=\mathcal{L}_i'(\phi_i)&&: i\text{-th gradient obtained during SGD}\\
%     \phi_{i+1}&=\phi_i-\alpha \cdot g_i&&: \text{sequence of parameter vectors}\\
%     \bar{g}_i&=\mathcal{L}_i'(\phi_0)&&: i\text{-th gradient at initial point}\\
%     \bar{H}_i&=\mathcal{L}_i''(\phi_0)&&: i\text{-th Hessian at initial point}\\
% \end{align*}

\subsection{Meta-gradient}
As shown in the Reptile~\cite{}, meta-gradient is $MG=\sum_{\tau \in \mathcal{T}}(\phi^\tau_k-\phi)$

\subsection{Reflection to inner steps}
Using meta-gradient, base parameter will be updated as $\theta\leftarrow\theta-\beta\cdot\textrm{MG}$. This movement of initial point will affect to parameter after $k$ steps, i.e. $\phi_k$, and we will approximate where the parameters should be moved, i.e. $\tilde\phi_k$,  using Taylor approximation. 
\begin{align}
    \tilde\phi_0 &= \phi_0 - \beta\cdot \textrm{MG} \\ 
    \tilde\phi_{1} &= \tilde\phi_0 - \alpha \cdot  \mathcal{L}_0'(\tilde\phi_0) \\
    \mathcal{L}_0'(\tilde\phi_0) &= \mathcal{L}_0'(\phi_0) + (\tilde\phi_0-\phi_0)\mathcal{L}_0''(\tilde\phi_0) + \mathcal{O}() \\  
\end{align}



==> sections/table1.tex <==
\begin{table*}[t]
\vspace{-0.05in}
\centering
\small
  \caption{\small\textbf{Test classification accuracies (\%) on various target datasets.} The reported numbers are the mean accuracies and standard deviations over 6 runs (2 meta-learned initializations $\times$ 3 task-specific runs).}
  \vspace{0.05in}
% \resizebox{1.\linewidth}{!}{
 \begin{tabular}{c |c c c c c c c}
 \hline
 & \multicolumn{6}{c}{Target Dataset} \\
 Model & Stanford Cars & STL10 & VGG Flowers & VGG Pets & DTD & QuickDraw \\
 \hline
 \hline
From scratch 
& 44.80\tiny$\pm$0.92 % Stanford Cars 
& 67.50\tiny$\pm$0.29 % STL10 
& 41.20\tiny$\pm$0.37 % VGG Flowers
& 63.04\tiny$\pm$0.54 % VGG Pets
& 43.93\tiny$\pm$1.17 % DTD
& 54.48\tiny$\pm$0.16 % QuickDraw
\\
% & 99.82\tiny$\pm$x.xx 

Finetuning (MTL) 
& 63.21\tiny$\pm$0.35 % Stanford Cars 
& 76.67\tiny$\pm$0.22 % STL10 
& 62.41\tiny$\pm$0.36 % VGG Flowers
& 74.98\tiny$\pm$0.91 % VGG Pets
& 53.34\tiny$\pm$0.54 % DTD
& 56.62\tiny$\pm$0.15 % QuickDraw
\\
% & xx.xx\tiny$\pm$x.xx

Finetuning (w/ TIN) 
& 64.47\tiny$\pm$0.68 % Stanford Cars 
& 77.39\tiny$\pm$0.24 % STL10 
& 65.88\tiny$\pm$0.44 % VGG Flowers
& 74.97\tiny$\pm$0.42 % VGG Pets
& 53.58\tiny$\pm$0.56 % DTD
& 56.97\tiny$\pm$0.10 % QuickDraw
\\
% & xx.xx\tiny$\pm$x.xx 

\hline

FOMAML~\cite{finn2017model}
& 44.66\tiny$\pm$1.01 % Stanford Cars 
& 69.30\tiny$\pm$0.48 % STL10 
& 41.11\tiny$\pm$0.80 % VGG Flowers
& 65.35\tiny$\pm$0.27 % VGG Pets
& 47.54\tiny$\pm$0.57 % DTD
& 55.23\tiny$\pm$0.20 % QuickDraw
\\
% & xx.xx\tiny$\pm$x.xx 


Leap~\cite{leap}
& 64.01\tiny$\pm$0.52 % Stanford Cars 
& 76.23\tiny$\pm$0.31 % STL10 
& 63.05\tiny$\pm$0.41 % VGG Flowers
& 73.74\tiny$\pm$0.56 % VGG Pets
& 52.32\tiny$\pm$0.60 % DTD
& 56.55\tiny$\pm$0.08 % QuickDraw
\\ 
% & xx.xx\tiny$\pm$x.xx 


Reptile~\cite{reptile}
& 67.66\tiny$\pm$0.47 % Stanford Cars 
& 78.81\tiny$\pm$0.21 % STL10 
& 68.74\tiny$\pm$0.80 % VGG Flowers
& 77.63\tiny$\pm$0.49 % VGG Pets
& 54.50\tiny$\pm$0.53 % DTD
& \bf 57.41\tiny$\pm$0.14 % QuickDraw
\\
% & xx.xx\tiny$\pm$x.xx 

\hline

\bf Ours
& \bf 68.22\tiny$\pm$0.60 % Stanford Cars 
& \bf 79.68\tiny$\pm$0.20 % STL10 
& \bf 69.33\tiny$\pm$0.41 % VGG Flowers
& \bf 79.43\tiny$\pm$0.53 % VGG Pets
& \bf 54.93\tiny$\pm$0.72 % DTD
& \bf 57.41\tiny$\pm$0.18 % QuickDraw
\\ 

%\bf Ours
%& $10^4$ & $5$
%& \bf xx.xx\tiny$\pm$x.xx % Stanford Cars 
%& \bf xx.xx\tiny$\pm$x.xx % STL10 
%& \bf xx.xx\tiny$\pm$x.xx % VGG Flowers
%& \bf xx.xx\tiny$\pm$x.xx % VGG Pets
%& \bf xx.xx\tiny$\pm$x.xx % DTD
%& \bf xx.xx\tiny$\pm$x.xx % QuickDraw
%\\ 

%\bf Leap + Ours
%& \bf xx.xx\tiny$\pm$x.xx % Stanford Cars 
%& \bf xx.xx\tiny$\pm$x.xx % STL10 
%& \bf xx.xx\tiny$\pm$x.xx % VGG Flowers
%& \bf xx.xx\tiny$\pm$x.xx % VGG Pets
%& \bf xx.xx\tiny$\pm$x.xx % DTD
%& \bf xx.xx\tiny$\pm$x.xx % QuickDraw
%\\ 
% & \bf xx.xx\tiny$\pm$x.xx 
\hline
\end{tabular}
%}

  \label{tbl:main}
  \vspace{-0.22in}
\end{table*}

==> sections/table2.tex <==
\begin{table*}[t]
\centering
\small
\vspace{-0.1in}
  \caption{\small\textbf{Test classification accuracies (\%).} The reported numbers are the mean accuracies and standard deviations over 3 runs.}
  \vspace{0.05in}
 \begin{tabular}{c | c c c c c c c}
 \hline
 & \multicolumn{6}{c}{Target Dataset} \\
 Model & Stanford Cars & Food 101 & Aircraft & CUB & VGG Flowers & VGG Pets \\
 \hline
 \hline
From scratch 
& xx.xx\tiny$\pm$x.xx % cars
& xx.xx\tiny$\pm$x.xx % food
& xx.xx\tiny$\pm$x.xx % aircraft
& xx.xx\tiny$\pm$x.xx % cub
& xx.xx\tiny$\pm$x.xx % flowers
& xx.xx\tiny$\pm$x.xx % pets
\\
ImageNet Finetuning
& xx.xx\tiny$\pm$x.xx % cars
& xx.xx\tiny$\pm$x.xx % food
& xx.xx\tiny$\pm$x.xx % aircraft
& xx.xx\tiny$\pm$x.xx % cub
& xx.xx\tiny$\pm$x.xx % flowers
& xx.xx\tiny$\pm$x.xx % pets
\\

ImageNet Finetuning + MTL
& xx.xx\tiny$\pm$x.xx % cars
& xx.xx\tiny$\pm$x.xx % food
& xx.xx\tiny$\pm$x.xx % aircraft
& xx.xx\tiny$\pm$x.xx % cub
& xx.xx\tiny$\pm$x.xx % flowers
& xx.xx\tiny$\pm$x.xx % pets
\\


\hline
\bf ImageNet Finetuning + Ours
& xx.xx\tiny$\pm$x.xx % cars
& xx.xx\tiny$\pm$x.xx % food
& xx.xx\tiny$\pm$x.xx % aircraft
& xx.xx\tiny$\pm$x.xx % cub
& xx.xx\tiny$\pm$x.xx % flowers
& xx.xx\tiny$\pm$x.xx % pets
\\

\hline
\end{tabular}

  \label{tbl:imagenet}
  \vspace{-0.15in}
\end{table*}

==> supp_figures/fig_landscape.tex <==
\begin{figure*}[t]
    \vspace{-0.05in}
	\centering
	\subfigure[$k=5$]{
	    \includegraphics[height=3.95cm]{figures/bar_5_6-min-2.png}
	    \label{fig:bar_5}
	}
	\subfigure[$k=100$]{
	    \includegraphics[height=3.95cm]{figures/bar_100_6-min-2.png}
	    \label{fig:bar_80}
	}
	\subfigure[Starting point: $(-5,5)$]{
	    \includegraphics[height=3.9cm]{figures/quality_phi1.pdf}
	    \label{fig:quality_phi1}
	}
	\subfigure[Starting point: $(5,-5)$]{
	    \includegraphics[height=3.9cm]{figures/quality_phi2.pdf}
	    \label{fig:quality_phi2}
	}
	\vspace{-0.17in}
	\caption{\small \textbf{(a,b) Meta-learning trajectories of Reptile} with the length of inner-optimization fixed as $k$. We collect the trajectories by initiating them from the various points in the grid of $\phi$ space. Meta-level local optima are shown by the red dots. \textbf{(c,d) Background contour: Task-average loss} after taking $100$ gradient steps from each point. The darker the better quality of the initialization point. \textbf{Lines: Meta-learning trajectories} of $\phi$ obtained from the baselines and our algorithm.  }
	\vspace{-0.1in}
    \label{fig:synthetic_figs2}
\end{figure*} 

==> supp_figures/fig_synthetic.tex <==
\begin{figure*}[t]
\vspace{-0.125in}
	\centering
	\subfigure[Template function]{
	    \includegraphics[height=3.6cm]{figures/loss_temp.pdf}
	    \label{fig:task}
	}
	\subfigure[Task $1$ loss function $\mathcal{L}^{(1)}$]{
	    \includegraphics[height=3.6cm]{figures/loss_task1.pdf}
	    \label{fig:task1}
	}
	\subfigure[Short horizon bias]{
	    \includegraphics[height=3.6cm]{figures/meta_loss_at_meta_optima.pdf}
	    \label{fig:largeK}
	}
	\subfigure[Computational cost]{
	    \includegraphics[height=3.5cm]{figures/thetable.pdf}
	    \label{fig:thetable}
	}
	\vspace{-0.17in}
	\caption{\small \textbf{(a)} Template function used to generate the task loss functions. \textbf{(b)} Task $1$ loss function $\mathcal{L}^{(1)}$ obtained by applying shift (black arrow) and random rotation. \textbf{(c)} Task-average loss after $100$ gradient steps from $\phi^*$ vs. $k$ used to obtain the optimal initialization parameters $\phi^*$ over the tasks.  \textbf{(d)} Computational cost in terms of total cumulative number of inner-gradient steps. }
    \label{fig:synthetic_figs1}
    \vspace{-0.125in}
\end{figure*} 

==> supp_figures/tbl_imageclassification.tex <==

%\input{sections/table1}

\begin{figure*}[t]
    \vspace{-0.15in}
	\centering
	\hspace{-0.1in}
	\hfill
	\subfigure[Meta-convergence]{
	    \raisebox{-0.05in}{
	    \includegraphics[height=3.8cm]{figures/metatrain.pdf}
	    \label{fig:meta_convergence}
	    }
	}
	\hspace{-0.2in}
	\hfill
	\subfigure[Meta-testing performance of the baselines]{
		\raisebox{-0.05in}{
	    \includegraphics[height=3.8cm]{figures/NEW6_bar.pdf}
	    \label{fig:bar}
	    }
	}
	\hspace{-0.2in}
	\hfill
	\subfigure[Stanford Cars]{
	    \raisebox{-0.05in}{
	    \includegraphics[height=3.8cm]{figures/NEW6_varyingK_cars.pdf}
	    \label{fig:varyingK_cars}
	    }
	}
	\hspace{-0.2in}
	\hfill
	\subfigure[Quickdraw]{
	    \raisebox{-0.05in}{
	    \includegraphics[height=3.8cm]{figures/NEW6_varyingK_quickdraw.pdf}
	    \label{fig:varyingK_quickdraw}
	    }
	}
	\hspace{-0.1in}
	\hfill
	%\subfigure[Test Acc. (Stanford Cars)]{
	%    \includegraphics[height=3.9cm]{figures/cars.pdf}
	%    \label{fig:convergence_cars}
	%}
	%\subfigure[Test Acc. (STL10)]{
	%    \includegraphics[height=3.9cm]{figures/stl10.pdf}
	%    \label{fig:convergence_stl10}
	%}
	%\subfigure[Test Acc. (VGG Flowers)]{
	%    \includegraphics[height=3.95cm]{figures/flower.pdf}
	%    \label{fig:convergence}
	%}
	\vspace{-0.15in}
	\caption{\textbf{(a) Meta-training convergence} measured as task-average training loss vs. cumulative inner-gradient steps.  \textbf{(b) Meta-testing performance} of the baselines. \textbf{(c) Meta-testing performance} vs. $K$ used for meta-training.}
	\vspace{-0.2in}
\end{figure*} 


\begin{figure*}[t]
	\centering
	\hspace{-0.2in}
	\hfill
	\subfigure[Stanford Cars]{
	    \raisebox{-0.05in}{
	    \includegraphics[height=3.8cm]{figures/NEW6_cars.pdf}
	    }
	}
	\hspace{-0.2in}
	\hfill
    \subfigure[Quickdraw]{
	    \raisebox{-0.05in}{
	    \includegraphics[height=3.8cm]{figures/NEW6_quickdraw.pdf}
	    }
	}
	\hspace{-0.2in}
	\hfill
	\subfigure[VGG Flowers]{
	    \raisebox{-0.05in}{
	    \includegraphics[height=3.8cm]{figures/NEW6_flower.pdf}
	    }
	}
	\hspace{-0.2in}
	\hfill
    \subfigure[VGG Pets]{
	    \raisebox{-0.05in}{
	    \includegraphics[height=3.8cm]{figures/NEW6_pets.pdf}
	    }
	}
	\hspace{-0.2in}
	\hfill
	\subfigure[STL10]{
	    \raisebox{-0.05in}{
	    \includegraphics[height=3.8cm]{figures/NEW6_stl10.pdf}
	    }
	}
	\hspace{-0.2in}
	\hfill
	\vspace{-0.15in}
	\caption{\textbf{Meta-testing performance} to show how efficient each method is in terms of cumulative inner-gradient steps spent for meta-training. We report mean and $95\%$ confidence intervals over $5$ runs. }
	\label{fig:new6}
	\vspace{-0.15in}
\end{figure*} 

==> supp_sections/imagenet.tex <==
\section{Improving on ImageNet Pre-trained Model}
\label{sec:imagenet_experiment}

    We demonstrate that our method is indeed capable of improving on the ImageNet finetuning under limited data regime. 
    
    \vspace{-0.05in}
    \paragraph{Datasets.} For \textbf{meta-training}, we construct a heterogeneous data distribution by class-wisely dividing the original ImageNet dataset into $8$ subsets based on the WordNet class hierarchy. We then meta-train the model over the obtained subsets. See Figure~\ref{fig:hierarchy} and Table~\ref{tbl:imagenet_split} for more information. For evaluation, we \textbf{meta-test} all methods with the $9$ benchmark image classification datasets described in Table~\ref{tbl:imagenet_dataset}. 
    
    
    \vspace{-0.05in}
    \paragraph{Experimental setup.} We use ResNet18~\cite{he2016deep}, which is suitable for the images of size $224\times 224$. We use random cropping and horizontal flipping as data augmentations. 
    \begin{itemize}
    \vspace{-0.05in}
    \item \textbf{Meta-training:} For MTL, Reptile and our model, we start from the ImageNet pretrained model for the meta-training to converge faster and reach a better solution than meta-training from scratch. We use SGD with momentum ($\mu=0.9$) as the inner-optimizer without applying the weight decay ($\lambda=0$). We set the batch size to $256$.  For \textbf{MTL}, we set the learning rate to $0.01$ and train for $50,000$ steps. For \textbf{Reptile} and \textbf{our model}, we use $\alpha=0.01$, $K=1,000$, and $M=50$, but use different meta-learning rate $\beta$ ($\beta=1$ for Reptile and $\beta=0.001$ for our model), since the optimal meta-learning rate differs across two methods. We meta-train for $50,000$ steps. 
    \vspace{-0.05in}
    \item \textbf{Meta-testing:} We subsample each target dataset such that each contains $1,000$ training datapoints. We normalize each input image with the mean and standard deviation of RGB channels across the whole training datapoints. We set the batch size to $256$. We train $K=1,000$ steps with Nesterov momentum optimizer ($\mu=0.9$). The starting learning rate is $\alpha=0.01$, and we step-wisely decay $\alpha$ at $400$, $700$, and $900$ steps by multiplying $0.2$. We use the weight decay $\lambda=0.0001$.
    \end{itemize}
    
    \begin{wrapfigure}{t}{0.23\linewidth}
	\centering
	%\vspace{-0.2in}
	\includegraphics[width=\linewidth]{supp_figures/metatrain3.pdf}
	\vspace{-0.35in}
	\caption{\small Meta-training convergence. }
	\vspace{-0.2in}
	\label{fig:convergence_scratch}
    \end{wrapfigure}
    
    \vspace{-0.05in}
    \paragraph{Results and analysis} Table~\ref{tbl:imagenet} shows the results. We empirically observe that our method is more effective when the task-specific learning suffers from overfitting. In order to clearly see this effect, we subsample each target dataset to contain only $1,000$ images and compare the performances. Table~\ref{tbl:imagenet} shows that our method consistently outperforms the baselines across most of the datasets when each target dataset has a limited number of instances. Figure~\ref{fig:imagenet_instances} confirms that on most of the target datasets, the performance improvements from the base ImageNet finetuning increase as the size of each dataset gets smaller. We conjecture that the performance improvements comes from the \emph{smoother} initial model parameter learned with our meta-learning algorithm, which may correspond to a stronger prior over the model parameters that can effectively regularize the task-specific learning with the small datasets. Lastly, Figure~\ref{fig:convergence_scratch} shows that also in this larger-scale experiments, our model converges much faster than Reptile when meta-training \emph{from scratch}. However, we found that the meta-testing from scratch yields worse performances than starting the meta-training from the ImageNet pretrained model.
    
    \input{sections/table2_re}
    
    
    %For Tiny ImageNet, we class-wisely divide the dataset into two smaller datasets. %Tasks for meta-training have a different number of classes and input size, which demonstrates heterogeneity. 
    %We then \textbf{meta-test} with $8$ datasets: \textbf{Food 101}~\cite{BossardGG14}, \textbf{Stanford Cars}, \textbf{Stanford Dogs}, \textbf{Aircraft}, \textbf{VOC2007}~\cite{pascal-voc-2007}, \textbf{VGG Flowers}, \textbf{CUB}, and \textbf{X-ray}.
    %STL10 is a benchmark classification dataset of general categories, and other datasets include fine-grained classification that may require large amount of task-specific ataptation (e.g. Stanford Cars), grey-scale images (QuickDraw), and texture dataset (DTD). For images bigger than $84 \times 84$, we resize the width and height of them into one of $\{28, 32, 64, 84\}$ for faster experiment. See the Appendix ... for more information.
    %\vspace{-0.12in}
    %\paragraph{Experimental setup} 
    %Then, we transfer meta-learnedinitialization, $\phi$, to several tasks. For every task, 
    %In this experiment we use ResNet18 which is suitable for images of size $224 \times 224$. See the Appendix for more information in detail.%For \textbf{meta-training}, we use $\alpha=0.01$, $\beta=0.1$, $K=1,000$, and $M=50$. We use SGD with Momentum ($\mu=0.9$) and weight decay ($\lambda=0.0005$) as the inner optimizer. For \textbf{meta-testing}, we train total $10,000$ steps for each dataset. We use Adam optimizer with $\alpha=0.001$, and $\lambda=0.0005$.
    %\vspace{-0.1in}
    %\paragraph{Results and analysis} TODO. s

==> supp_sections/table2.tex <==
\begin{table}[H]
\centering
\small
  \caption{\small\textbf{Test classification accuracies (\%)} when we let each target dataset contain only 1,000 images. We report the mean accuracies and the $95\%$ confidence intervals over 5 runs.}
  \vspace{0.05in}
  \resizebox{1.\linewidth}{!}{
 \begin{tabular}{c | c c c c c c c c c c}
 \hline
  ImageNet & \multicolumn{8}{c}{Target dataset} \\
pre-training & Dogs & Cars & Pets & Flowers & Food-101 & Aircraft & CUB & SUN397 & DTD \\
 \hline
 \hline
+ None
& 55.56\tiny$\pm$0.29 % dogs
& 23.15\tiny$\pm$0.27 % cars
& 83.48\tiny$\pm$0.15 % pets
& 87.01\tiny$\pm$0.38 % flowers
& 36.95\tiny$\pm$0.37 % food
& 33.43\tiny$\pm$0.29 % aircraft
& 34.32\tiny$\pm$0.46 % cub
& 29.62\tiny$\pm$0.24 % sun
& 59.39\tiny$\pm$0.53 % dtd
\\

+ MTL
& 55.00\tiny$\pm$0.28 % dogs
& \bf 23.82\tiny$\pm$0.19 % cars
& 83.29\tiny$\pm$0.25 % pets
& 87.04\tiny$\pm$0.34 % flowers
& 36.84\tiny$\pm$0.37 % food
& 34.02\tiny$\pm$0.55 % aircraft
& 34.19\tiny$\pm$0.88 % cub
& 29.30\tiny$\pm$0.28 % sun
& 58.86\tiny$\pm$0.49 % dtd
\\

+ Reptile
& 56.97\tiny$\pm$0.12 % dogs
& 22.49\tiny$\pm$0.40 % cars
& 84.25\tiny$\pm$0.22 % pets
& 87.22\tiny$\pm$0.31 % flowers
& 37.35\tiny$\pm$0.22 % food
& 33.81\tiny$\pm$0.35 % aircraft
& 35.44\tiny$\pm$0.48 % cub
& 29.37\tiny$\pm$0.29 % sun
& 58.98\tiny$\pm$0.59 % dtd
\\

\hline
\bf + Ours
& \bf 57.53\tiny$\pm$0.48 % dogs
& 23.80\tiny$\pm$0.40 % cars
& \bf 84.65\tiny$\pm$0.11 % pets
& \bf 87.54\tiny$\pm$0.21 % flowers
& \bf 37.84\tiny$\pm$0.20 % food
& \bf34.42\tiny$\pm$0.48 % aircraft
& \bf 36.40\tiny$\pm$0.20 % cub
& \bf 29.74\tiny$\pm$0.08 % sun
& \bf 59.53\tiny$\pm$0.25 % dtd

\\

\hline
\end{tabular}
}

  \label{tbl:imagenet}
  \vspace{-0.15in}
\end{table}

==> supp_sections/table2_re.tex <==
\begin{table}[t]
\centering
\small
  \caption{\small\textbf{Classification accuracies obtained with various pre-training methods (\%)} when the target dataset contains 1,000 images. We report the mean accuracies and the $95\%$ confidence intervals over 5 runs.}
  \vspace{0.05in}
  \resizebox{1.\linewidth}{!}{
 \begin{tabular}{c | c c c c c c c c c |c}
 \hline
  ImageNet & \multicolumn{9}{c|}{Target dataset} & \\
pre-training & CIFAR100 & CIFAR10 & SVHN & Dogs & Pets & Flowers & Food & CUB & DTD & Avg.\\
 \hline
 \hline
+ None
& 41.95\tiny$\pm$0.29 % cifar100
& 81.60\tiny$\pm$0.28 % cifar10
& 60.09\tiny$\pm$0.98 % svhn 
& 55.56\tiny$\pm$0.29 % dogs
& 83.48\tiny$\pm$0.15 % pets
& 87.01\tiny$\pm$0.38 % flowers
& 36.95\tiny$\pm$0.37 % food
& 34.32\tiny$\pm$0.46 % cub
& 59.39\tiny$\pm$0.53 % dtd
& 60.04
\\

+ MTL
& 42.79\tiny$\pm$0.54 % cifar100
& 82.33\tiny$\pm$0.20 % cifar10
& 59.05\tiny$\pm$1.09 % svhn 
& 55.00\tiny$\pm$0.28 % dogs
& 83.29\tiny$\pm$0.25 % pets
& 87.04\tiny$\pm$0.34 % flowers
& 36.84\tiny$\pm$0.37 % food
& 34.19\tiny$\pm$0.88 % cub
& 58.86\tiny$\pm$0.49 % dtd
& 59.93
\\

+ Reptile
& 47.98\tiny$\pm$0.14 % cifar100
& \bf 84.58\tiny$\pm$0.12 % cifar10
& 62.39\tiny$\pm$0.72 % svhn 
& 56.97\tiny$\pm$0.12 % dogs
& 84.25\tiny$\pm$0.22 % pets
& 87.22\tiny$\pm$0.31 % flowers
& 37.35\tiny$\pm$0.22 % food
& 35.44\tiny$\pm$0.48 % cub
& 58.98\tiny$\pm$0.59 % dtd
& 61.68
\\

\hline
\bf + Ours
& \bf 48.34\tiny$\pm$0.21 % cifar100
& 84.42\tiny$\pm$0.15 % cifar10
& \bf 62.82\tiny$\pm$0.56 % svhn 
& \bf 57.53\tiny$\pm$0.48 % dogs
& \bf 84.65\tiny$\pm$0.11 % pets
& \bf 87.54\tiny$\pm$0.21 % flowers
& \bf 37.84\tiny$\pm$0.20 % food
& \bf 36.40\tiny$\pm$0.20 % cub
& \bf 59.53\tiny$\pm$0.25 % dtd
& \bf 62.12

\\

\hline
\end{tabular}
}

  \label{tbl:imagenet}
  \vspace{-0.15in}
\end{table}

\begin{figure}[t]
    \vspace{-0.05in}
	\centering
	\hfill
	\subfigure[CIFAR100]{
	    \includegraphics[height=3.8cm]{figures/FT_cifar100.pdf}
	}
	\hfill
	\subfigure[SVHN]{
	    \includegraphics[height=3.65cm]{figures/FT_svhn.pdf}
    }
	\hfill
	\subfigure[Pets]{
	    \includegraphics[height=3.65cm]{figures/FT_pets.pdf}
    }
	\hfill
	\subfigure[Food]{
	    \includegraphics[height=3.65cm]{figures/FT_food.pdf}
    }
	\hfill
	\subfigure[CUB]{
	    \includegraphics[height=3.65cm]{figures/FT_cub.pdf}
    }
	\hfill
	\vspace{-0.15in}
	\caption{\small Performance improvements (Accuracy, \%) over ImageNet Finetuning. }
	\vspace{-0.05in}
    \label{fig:imagenet_instances}
\end{figure} 
